QUINT: Node embedding using network hashing

Representation learning using network embedding has received tremendous attention due to its efficacy to solve downstream tasks. Popular embedding methods (such as deepwalk, node2vec, LINE) are based on a neural architecture, thus unable to scale on large networks both in terms of time and space usage. Recently, we proposed BinSketch, a sketching technique for compressing binary vectors to binary vectors. In this paper, we show how to extend BinSketch and use it for network hashing. Our proposal named QUINT is built upon BinSketch, and it embeds nodes of a sparse network onto a low-dimensional space using simple bi-wise operations. QUINT is the first of its kind that provides tremendous gain in terms of speed and space usage without compromising much on the accuracy of the downstream tasks. Extensive experiments are conducted to compare QUINT with seven state-of-the-art network embedding methods for two end tasks - link prediction and node classification. We observe huge performance gain for QUINT in terms of speedup (up to 7000x) and space saving (up to 80x) due to its bit-wise nature to obtain node embedding. Moreover, QUINT is a consistent top-performer for both the tasks among the baselines across all the datasets. Our empirical observations are backed by rigorous theoretical analysis to justify the effectiveness of QUINT. In particular, we prove that QUINT retains enough structural information which can be used further to approximate many topological properties of networks with high confidence.

==> Analysis.tex <==
 \section{Analysing \texttt{QUINT}}\label{sec:analysis}
 
\newcommand{\bs}{{\tt EstCN}\xspace}
\newcommand{\IPS}[1]{\langle #1 \rangle}
\newcommand{\hatn}{\hat{n}}
\newcommand{\hatd}{\hat{\delta}}

In this section we analyse the theoretical properties of \quint that make it suitable for embedding graphs, especially for link prediction and node classification. It will be easy to remember that the embedding of a node $i$ is a $d$-dimensional binary vector which is denoted $\sigma_i$ and is defined as\\
\centerline{$\mbox{ $j$-th coordinate of $\sigma_i$: } = (\sigma_i)_j  = \bigvee_{k: \pi(k)=j} A_{ik}$}
where $\pi$ denotes a random mapping from $\{1, 2, 3, \ldots, n\}$ to $\{1, 2, 3, \ldots, d\}$ and $A$ denotes the adjacency matrix.

 %In this section, we explain our embedding technique \texttt{QUINT}, discuss the properties of a graph it seeks to preserve and explain a few attractive features that make it suitable for embedding graphs, especially for link prediction and node classification.
 
 %The idea behind {\tt QUINT} has its seed in the \texttt{BinSketch} hashing technique and an algorithm to estimate inner products of binary vectors from their hashes~\cite{binsketch_arxiv}. However, we heavily modify it to obtain important theoretical guarantees.
 
\subsection{Time and space complexity}

The random mapping can be generated once and stored as a fast-lookup table or can be implemented using an efficient hashing algorithm. Let $S$ denote the space required and $T$ denote the time-complexity to compute $\pi(\cdot)$; for a lookup table stored in RAM, $S = O(n \log d)$ and $T = O(1)$. Apart from the overhead of $\pi$, \texttt{QUINT} only involves bit manipulations which makes it extremely efficient. We assume that $G$ is stored as an adjacency list (which has asymptotically same space complexity as that of an edge-list representation).

\begin{lemma}
Algorithm~\ref{algo:QUINT} runs in time $\Theta(T \cdot |E|)$, returns an embedding using $d \cdot |V|$ bits and requires an additional space $S$ for the embedding.
\end{lemma}

The node embeddings too can be stored in RAM; we observe that $\pi$ need not be stored once a graph is embedded. Another alternative is to not store the embedding, store only $\pi$ and generate $\sigma_i$ on demand --- this approach is also efficient given the lightweight embedding algorithm.

\begin{lemma}
 The embedding of a single node  $i$ uses only $d$ bits and can be computed in time $O(T \cdot n(i))$, where $n(i)$ denotes the degree of $i$, and without any additional space overhead.% The internal space required is to store the random mapping $\pi$.
\end{lemma}

Taking $T$ and $d$ to be constant for practical scenarios, both these approaches take constant time per edge of the network and use constant space per node of the network.

% The above lemma ensures that our embedding algorithm is update friendly. That is, suppose we have a dynamic graph on $n$ nodes whose embedding $\{\sigma_1, \sigma_2, \ldots, \sigma_n\}$ is already computed, and now, an edge $(i,j)$ is added to the graph. The embedding of the updated graph can be efficiently computed by using $L = \{(i,j), ~(j,i)\}$ in Line~\ref{line:QUINT1} of Algorithm~\ref{algo:QUINT}.

% Matrix operations are naturally adaptable to distributed settings and so is the case for {\tt QUINT}; embedding of each node can be computed indepedently of the others in a completely parallel and distributed manner. In fact, tabulation hashing techniques can be used to distribute the mapping function as well and one can even distribute the computation on the basis of dimensions.

\subsection{Estimating number of neighbors}
The {\em number of neighbors} of a node can be easily estimated from its embedding by adapting a result that was proved along with $\binsketch$~\cite{binsketch} except that we use a larger $d$ compared to what was used there.

%     \begin{algorithm}
%     \begin{flushleft}
% 	\hspace*{\algorithmicindent} \textbf{Input:} Embedding $\sigma_i$ of $i$\\
% 	\hspace*{\algorithmicindent} \textbf{Parameter:} Embedding dimension $d$
% 	\end{flushleft}
% 	\begin{algorithmic}[1]
% 	    \State Compute $\hatn^s_{i}=|\sigma_i|$ \Comment{$|v|$: number of ones in vector $v$}
% 	    \If{$\hatn^s_{i}=0$}
% 	        \State \Return $\hatn_i=0$ \label{line:algoestn-sp-case}
% 	    \EndIf
% 	    \State \Return $\hatn_i=\ln(1-\frac{\hatn^s_i}{d})/\ln(D)$ \Comment{$D$ denotes $1-\frac{1}{d}$}
% 	\end{algorithmic}
% 	\caption{{\tt EstN} (number of neighbors of node $i$)\label{algo:estn}}
%     \end{algorithm}
    
%The {\tt EstN} algorithm (Algorithm~\ref{algo:estn}) was proposed recently~\cite{binsketch_arxiv}, and there it was shown that it gives a good approximation of the number of neighbors of a node, i.e., its degree.
    
\begin{lemma}[\cite{binsketch}, Lemma 8]
There is a linear-pass algorithm to estimate the number of neighbors of a node $i$ with at most $4\sqrt{\frac{\psi}{2}\ln \frac{2}{\delta}}$ additive inaccuracy and probability at least $1-\delta$.
\end{lemma}

\subsection{Estimating number of common neighbors}
The first-order proximity between nodes $i$ and $j$ is an indicator denoting the presence of an edge between them. \quint, in its current form, does not preserve the first-order proximity. Surprisingly, \quint\ allows us to estimate the second-order proximity for a common similarity measure used for node classification and prediction: the {\em similarity} of two nodes, say $i$ and $j$, by the number of their common neighbors, denoted $n_{i,j}$.  Note that $n_{i,j} \le \psi$, degree of the graph. We describe the technique in Algorithm~\ref{algo:bs}) and the corresponding result in Theorem~\ref{thm:binsketch}.


    \begin{algorithm}
    \begin{flushleft}
	\hspace*{\algorithmicindent} \textbf{Input:} embeddings $\sigma_i$ of $i$ and $\sigma_j$ of $j$\\
	\hspace*{\algorithmicindent} \textbf{Parameter:} embedding dimension $d$
	\end{flushleft}
	\begin{algorithmic}[1]
	    \State Compute $\hatn^s_{i}=|\sigma_i|$ \Comment{$|v|$: number of ones in vector $v$}
	    \State Compute $\hatn^s_j=|\sigma_j|$
	    \State Compute $\hatn^s_{i,j}=\IPS{\sigma_i, \sigma_j}$ \Comment{$\IPS{u,v}$: inner prod. of $u$ and $v$}
	    \If{$\hatn^s_{i,j}=0$}
	        \State \Return $\hatn_{i,j}=0$ \label{line:algobs-sp-case} \Comment{Enhancement from $\binsketch$}
	    \EndIf
	    \State Set $\hatn_i=\ln(1-\frac{\hatn^s_i}{d})/\ln(D)$ \Comment{$D$ denotes $1-\frac{1}{d}$}
	    \State Set $\hatn_j =\ln(1-\frac{\hatn^s_j}{d})/\ln(D)$
	    \State \Return estimated number of common neighbors $$\hatn_{i,j} = \hatn_i + \hatn_j - \tfrac{1}{\ln D} \ln
		\left(D^{\hatn_i}+D^{\hatn_j}+\frac{\hatn^s_{i,j}}{d}-1 \right)$$ 
	\end{algorithmic}
	\caption{\bs (number of common neighbors $n_{i,j}$)\label{algo:bs}}
    \end{algorithm}

% This can be observed from the \bs algorithm that is described in Algorithm~\ref{algo:bs}).
% that has an important modification in Line~\ref{line:algobs-sp-case} to the \texttt{BinSketch} algorithm proposed earlier~\cite[Algorithm 1]{binsketch}. The latter algorithm was designed to estimate the inner product of two binary vectors from their sketches, and we adapt it for estimating the number of common neighbors of any two distinct vertices from their embeddings. Adapting a result from \texttt{BinSketch}~\cite[Theorem 1]{binsketch} for our scenario, we show that the embedding produced by \texttt{QUINT} can be used, via the \bs algorithm, to produce a tight estimate of the number of common neighbors.

\begin{theorem}\label{thm:binsketch}
Let $\psi$ be an upper bound on the degree of $G$ and $\rho$ be the desired probability of error. If the embedding dimension $d$ is chosen as $\psi^2 \sqrt{\frac{\psi}{2} \ln \frac{2}{\rho}}$, then \bs ensures that its output satisfies the following with probability $\ge 1-\rho$.
$$n_{i,j} - 14\sqrt{\frac{\psi}{2} \ln \frac{6}{\rho}} \quad  <   \hatn_{i,j}  < \quad n_{i,j} + 14\sqrt{\frac{\psi}{2} \ln \frac{6}{\rho}}$$
Furthermore, 
\noindent\begin{enumerate}
\item if $n_{i,j} > 0$ then $\hatn_{i,j} > 0$, and
\item if $n_{i,j}=0$ then $\hatn_{i,j}=0$ with probability at least $1- \sqrt{2/(\psi \ln \tfrac{2}{\rho})}$.
\end{enumerate}
\end{theorem}

\noindent{\bf Enhancements to $\mathbf{\binsketch}$:} We quickly discuss how we modify $\binsketch$ to suit node embedding. The first part about the accuracy of $\bs$ in Theorem~\ref{thm:binsketch} is known as a feature of the \texttt{BinSketch} algorithm~\cite[Theorem 1]{binsketch}; however, in that algorithm the embedding dimension was set to $\psi \sqrt{\frac{\psi}{2} \ln \frac{2}{\rho}}$. Our first modification is a larger value $\psi^2\sqrt{\frac{\psi}{2} \ln \frac{2}{\rho}}$; observe that as the embedding dimension is increased, there are even lesser chances of collision in the computation of $\pi(\cdot)$ and higher chances of a particular bit of an encoding being set by only one bit of a source vector. Intuitively speaking, this will only result in better accuracy and lower probability of error in estimation compared to the \texttt{BinSketch} algorithm, but there is more.

The second part says that, with high probability, $n_{i,j}=0$ iff $\hatn_{i,j}=0$. This is important, since otherwise, the {\em estimated} number of common neighbors of $i$ and $j$ could be as large as $14\sqrt{\frac{\psi}{2} \ln \frac{6}{\rho}}$ even when $i$ and $j$ share no common neighbor.  The enhancement in Line~\ref{line:algobs-sp-case} of Algorithm~\ref{algo:bs} is crucial to prove the second part. Both of the modifications are neither cosmetic nor heuristic but are necessary to prove Theorem~\ref{thm:binsketch}, especially the second part. The importance of Theorem~\ref{thm:binsketch} is its role in concentrating $\hatn_{i,j}$ around the true value, and this enables us to prove Theorem~\ref{theorem:a4-approx} which says that certain higher order proximity are preserved by \quint.

\begin{proof}[Proof of second part]
For the first claim observe that if $n_{i,j} > 0$, then there must be some $k$ such that $A_{ik}=A_{jk}=1$. Let $t$ denote $\pi(k)$; then both $(\sigma_i)_t=(\sigma_j)_t$ will be set to 1. Thus, $\hatn^s_{i,j} = \IPS{\sigma_i,\sigma_j} > 0$. By way of contradiction, assume that $\hatn_{i,j} = 0$. But then we would see, from Algo.~\ref{algo:bs}, we have
\begin{comment}
\begin{align*}
    & & \mbox{(from Algo.~\ref{algo:bs})}\quad
    \hatn_i + \hatn_j & = \tfrac{1}{\ln D} \ln
		\left(D^{\hatn_i}+D^{\hatn_j}+\frac{\hatn^s_{i,j}}{d}-1 \right)\\
		&\equiv & D^{\hatn_i} \cdot D^{\hatn_j} & = D^{\hatn_i} + D^{\hatn_j} + \frac{\hatn^s_{i,j}}{d} - 1 \\
		&\equiv & \left(1 - \frac{\hatn^s_i}{d} \right) \left(1 - \frac{\hatn^s_j}{d} \right) & = \left(1 - \frac{\hatn^s_i}{d} \right) + \left(1 - \frac{\hatn^s_j}{d} \right) + \frac{\hatn^s_{i,j}}{d} - 1\\
		&\equiv & \frac{\hatn^s_i \cdot \hatn^s_j}{d^2} & = \frac{\hatn^s_{i,j}}{d}
\end{align*}
\end{comment}
\begin{align*}
  \hatn_i + \hatn_j & = \tfrac{1}{\ln D} \ln
		\left(D^{\hatn_i}+D^{\hatn_j}+\frac{\hatn^s_{i,j}}{d}-1 \right)\\
	  D^{\hatn_i} \cdot D^{\hatn_j} & = D^{\hatn_i} + D^{\hatn_j} + \frac{\hatn^s_{i,j}}{d} - 1 \\
	  \left(1 - \frac{\hatn^s_i}{d} \right) \left(1 - \frac{\hatn^s_j}{d} \right) & = \left(1 - \frac{\hatn^s_i}{d} \right) + \left(1 - \frac{\hatn^s_j}{d} \right) + \frac{\hatn^s_{i,j}}{d} - 1\\
	  \frac{\hatn^s_i \cdot \hatn^s_j}{d^2} & = \frac{\hatn^s_{i,j}}{d}
\end{align*}
The last identity is not true in general. For example, consider a scenario in which $\sigma_i \sim \sigma_j$ with the number of ones in each much less than $d$; in this case $|\sigma_i| \approx |\sigma_j| \approx \IPS{\sigma_i, \sigma_j}$ and $|\sigma_i| \ll d$, thus contradicting the identity.

For proving the second claim, take any $i$ and $j$ such that $n_{i,j}=0$, i.e., there is no $k$ such that both $A_{i,k}=A_{j,k}=1$. For the sake of contradiction, assume that $\hatn_{i,j} > 0$, i.e.,  there is some $t$ such that $(\sigma_i)_t = (\sigma_j)_t = 1$; this means that there must be some $k_1$ and $k_2$ such that $A_{i,k_1}=A_{j,k_2} = 1$ and $\pi(k_1)=\pi(k_2)=t$. The probability for the latter event, denoted $E$, is same as the probability that in a group of $n$ men and $n$ women, there exists at least one pair with a common birthday, which can be shown to be $$1 - \sum_{k=1}^M {D \choose k} k! \, S_{M,k} (D-k)^F/D^{F+M}$$
in which $S_{M,k}$ denotes Stirling's number of the second kind~\cite{stackxch-birthday}. Getting a closed form of this is difficult; therefore we show a different technique of bounding the probability of $E$.

Let $E_x$ be the event that $(\sigma_i)_x= (\sigma_j)_x=1$. It can be shown that $\E(E_x) =  \left(1-D^{|A_i|}\right) \cdot \left(1-D^{|A_j|}\right)$~\cite[Lemma 5]{binsketch}. Since $|A_i|$ and $|A_j|$ are both at most $\psi$, and $D < 1$, 
$$\E(E_x) \le (1-D^{\psi})^2 = \left(1 - \left(1-\frac{1}{d}\right)^{\psi}\right)^2 \le \left(\frac{\psi}{d}\right)^2$$
which implies that $\E[\sum_x E_x] = d\left(\frac{\psi}{d}\right)^2 = \frac{\sqrt{2}}{\sqrt{\psi\ln \frac{2}{\rho}}} \ll 1$

Let $E_{all}$ denote $\sum_x E_x$; $E_{all}$ is a random variable that denotes the number of positions $x$ such that $(\sigma_i)_x=(\sigma_j)_x=1$ and whose expectation we computed above. Since $E$ is equivalent to ``$E_{all} \ge 1$'', we apply Markov's inequality to derive an upper bound: $$\Pr[\hatn_{i,j} > 0] = \Pr[E] = \Pr[E_{all} \ge 1] \le \E[E_{all}] = \frac{\sqrt{2}}{\sqrt{\psi\ln \frac{2}{\rho}}}.$$
\end{proof}

For the rest of this section we will use the fact that \bs estimates non-zero $n_{i,j}$ values with a small additive error and accurately identifies $n_{i,j}=0$ values (both of these happen with non-negligible probability which we would not explicitly state for the sake of brevity).

% The authors of BinSketch claimed that $\psi \ge 20$ and $\rho < 0.1$ is required for the above bounds to hold; however, upon closer inspection of the proofs we found that $\psi \ge 4$ and $\rho < 0.1$ is sufficient. Moreover, $\psi$ should only be an upper bound of the degree. Hence, Theorem~\ref{thm:binsketch} is applicable to any graph whose degree can be bounded and this includes all the the sparse real-world graphs. {\color{red} do we perform experiments on dense graphs?}

\renewcommand{\L}{\mathcal{L}}

The above theorem allows us to accurately quantify the loss function ({\it aka.} objective function) that is used by most node embedding algorithms to {\em learn} the embedding~\cite{HamiltonYL17}. Using the mean-squared-error (MSE) to compute the loss function, we can represent it as
$$\L = \frac{1}{T}\sum_{(i,j) \in T \subseteq V \times V} | n_{i,j} - \bs(i,j) |^2.$$
Here $T$ represents a ``training set of edges'' that is traditionally used to learn an embedding. Our proposed technique does not involve any learning; nevertheless, for the sake of comparison we present an explicit upper bound on $\L$ --- it follows directly from Theorem~\ref{thm:binsketch}.

\begin{lemma}
Using \texttt{QUINT} for embedding and \bs for estimating node similarity, $\L$ is upper bounded by $196 \frac{\psi}{2} \ln \frac{6}{\rho}$.
\end{lemma}

\subsection{Estimating higher-order proximities}

Many node embedding algorithms operate on the paths, often up to a certain length, on a graph. For example, both the random-walk based approaches \texttt{deepwalk} and \texttt{node2vec} consider two nodes to be similar if their presence in short random walks on the graph is highly correlated. Here we show that \texttt{QUINT} also ``preserves'' path information in a certain manner. The key observation here is that the square of the adjacency matrix exactly contains the $n_{ij}$ values.

\begin{obs}
For any $i,j$, $A^2_{i,j} = n_{i,j}$.
\end{obs}
This is since $\sum\limits_{k = 1}^{n} A_{ik} A_{kj} = | \{ k \in V ~:~ (i, k) \in E,~ (k, j) \in E\}|$.

This observation along with Theorem~\ref{thm:binsketch} implies that \bs can approximately compute $A^2$.

\begin{lemma}\label{lemma:approx_A2}
$\bs(\sigma_i,\sigma_j)$ approximately computes $A^2_{i,j}$ with a small additive error. If $A^2_{i,j}=0$ $\bs(\sigma_i,\sigma_j)$ outputs 0.
\end{lemma}

Next we show how to translate the above lemma to higher {\em even} powers of $A$. We first show the result for the $4$-th power, $A^4$, each of whose entry, say $A^4_{i,j}$, denotes the number of paths between $i$ and $j$ using 4 nodes (and 3 edges).

We use $\epsilon_2$ to denote the small additive error mentioned in Lemma~\ref{lemma:approx_A2}. To maintain consistency of notations, we will use $\hatn2_{i,j}$ to denote $\hatn_{i,j}$; by construction, $\hatn2$ is symmetric.

\begin{theorem}\label{theorem:a4-approx}
Let $\hatn4_{i,j}$ denote the expression $\sum_{k=1}^n \hatn2_{i,k} \cdot \hatn2_{k,j}$ for all $i,j=1 \ldots n$. Then
$\hatn4_{i,j}$ approximately computes $A^4_{i,j}$ with a small additive error. If $A^4_{i,j}=0$ then $\hatn4_{i,j}$ outputs 0.
\end{theorem}

\begin{proof} Recall that $A^4_{i,j} = \sum_{k=0}^n A^2_{i,k} A^2_{k,j} = \sum_{k=0}^n A^2_{i,k} A^2_{j,k}$, and further more, each term in the summation is non-negative.
Therefore, $A^4_{i,j}=0$ implies that $A^2_{i,k}=0$ and $A^2_{j,k}=0$ for every $k=1 \ldots n$. We know from Lemma~\ref{lemma:approx_A2} that, in this case, $\hatn2_{i,k}=0$ and $\hatn2_{j,k}=0$ for all $k$. Clearly, $\hatn4^{i,j}=0$ too --- this proves the second part of the theorem.

For the first part, take any $i,j$ such that $A^4_{i,j} > 0$. That is, $\sum_{k=1}^n A^2_{i,k} A^2_{j,k} > 0$. 
From Lemma~\ref{lemma:approx_A2} we know that, for any $y$ and $x=i,j$, $|\hatn2_{x,y} - A^2_{x,y}| \le \epsilon_2$; using $z$ to denote the left-hand side, we can write $\hatn2_{x,y} = A^2_{x,y} + z$ where $-\epsilon_2 \le z \le \epsilon_2$ and 
$$\hatn4_{x,y} = \sum_{u=1}^{n} \hatn2_{x,u} \cdot \hatn2_{y,u}$$
We will use a technical result about $A$.
\begin{claim}\label{claim:1}
$\sum_{u=1}^n A^2_{x,u} \le \psi^2$.
\end{claim}
\begin{subproof}
$\psi$ being an upper bound on the degree of any node, the total number of length-2 paths from $x$ is at most $\psi^2$. $A^2_{x,u}$ is the total number of length-2 paths from $x$ to $u$ and $\sum_{u} A^2_{x,u}$ is the total number of length-2 paths from $x$ to any node, which is, therefore, upper bounded by $\psi^2$.
\end{subproof}
The next observation is applicable to sparse graphs in general but immensely beneficial to graphs where $\psi^2 \ll n$.
\begin{obs}\label{obs:2}
Since the entries of $A^2_{x,u}$ are non-negative, Claim~\ref{claim:1} implies that at most $\psi^2$ entries are non-zero in the $x$-th row of $A^2$, i.e, among $A^2_x = \{ A^2_{x,u} ~:~ u \in \{1, 2, \ldots, n\} \}$. That is, at least $n-\psi^2$ entries of $A^2_x$ are zero.
\end{obs}

This observation, along with Lemma~\ref{lemma:approx_A2}, implies that for any $x$, at most $\psi^2$ values in the set $\{\hatn2_{x,u} ~:~ u \in \{1, 2, \ldots n\} \}$ are non-zero. We use $(\sum_{u=1}^n)^{\le \psi^2}$ to denote the fact that in a summation with $n$ summands, at most $\psi^2$ terms are non-zero. Getting back to proving the theorem,
\begin{align*}
    \hatn4_{x,y}
    = & (\sum_{u=1}^n)^{\le \psi^2} (A^2_{x,u} + z) \cdot (A^2_{y,u} + z)\\
    = & \sum_{u=1}^n A^2_{x,u} \cdot A^2_{y,u} + z \cdot \sum_{u=1}^n A^2_{x,u} \\
    & + z \cdot \sum_{u=1}^n A^2_{y,u} + (\sum_{u=1}^n)^{\le \psi^2} z^2 \\
    = & A^4_{x,y} + 2z\psi^2 + z^2 \psi^2 \tag*{(Using Claim~\ref{claim:1})}
\end{align*}
Thus we get, $$\big|\hatn4_{x,y} - A^4_{x,y}\big| = \big|2z + z^2\big| ~ \psi^2 = \left\{
\begin{array}{ll}
    3|z|\psi^2 & \mbox{ if $|z| < 2$}\\
    2z^2 \psi^2 & \mbox{ if $|z| \ge 2$}
\end{array} \right.$$
Since $|z| \le \epsilon_2$ and the additive error $\epsilon_2$ for $\hatn^2_{x,y}$ is $\tilde{O}(\sqrt{\psi})$ from Theorem~\ref{thm:binsketch} (here $\tilde{O}()$ hides $\log(1/\rho)$ factors), so both $|z|,z^2$ is $\tilde{O}(\psi)$. Therefore, the additive error for $\hatn4_{x,y}$ is $\tilde{O}(\psi^3)$.
\end{proof}

Theorem~\ref{theorem:a4-approx} can be generalized to show that entries of $A^{2^t}$, for $t \ge 1$, can be approximated with additive error $\tilde{O}(poly(\psi))$. Since any even power of $A$ can be written as a product of $A$ raised to a power of 2, we have established that our \texttt{QUINT} embedding effectively preserves all even power of the adjacency matrix $A$, and therefore, can approximate information about paths of even lengths in $G$. 

==> Reproducibility.tex <==
\section{Reproducibility}\label{sec:reproducibility}
\noindent\textbf{Details on the candidate algorithms:}
For \texttt{node2vec}, we used the implementation provided by its authors \footnote{https://github.com/aditya-grover/node2vec}. We did a grid search over its parameters $p$ and $q \in [0.25, 0.5, 1, 2, 4]$, which  is equivalent to running $25$ different experiments.  We only 
 report the result for the optimum choice of $p$ and $q$. \texttt{deepwalk} is a special case of  \texttt{node2vec} when $p=q=1$~\cite{node2vec}, so the earlier {\tt node2vec} implementation was used here with the specified parameters. For \texttt{LINE}, we used a standard  implementation available online 
\footnote{\url{https://github.com/shenweichen/GraphEmbedding}} and performed experiments considering both first and second order proximity --- and report the   best result. \texttt{VERSE}~\cite{verse} \footnote{\url{https://github.com/xgfs/verse}} uses the idea of personalised PageRank to compute the embedding of nodes. 
%directly samples node pairs to learn graph embeddings to preserve the node proximity measured by personalizedPageRank. 
%We tune the damping factor $\alpha$ of personalized PageRank using the method suggested by the authors, and  we leave all
%other parameters as default.
\texttt{NetMF}~\cite{netmf}\footnote{\url{https://github.com/xptree/NetMF}} unifies the idea of sampling based algorithms such as \texttt{node2vec, deepwalk, LINE} in the  matrix factorisation framework and generate the embedding. % We tune the implicit window size $T$ within $\{1, 10\}$ suggested by the authors.
 \texttt{NodeSketch}~\cite{nodesketch}\footnote{\url{https://github.com/eXascaleInfolab/NodeSketch}} built on top of an efficient sketching technique and output embedding which preserve higher-order proximity via recursive approach. %As suggested by the authors, we search the optimal order of proximity up to $6$ and the optimal decay parameter $\alpha$ from $0.0001$ to $1$ on a $\log$ scale.
 \texttt{SGH}~\cite{sgh}\footnote{\url{4https://github.com/jiangqy/SGH-IJCAI2015}} learns the binary embedding of the nodes by minimizing the difference between the similarity of pair of nodes and hamming similarity of the corresponding binary hash codes.
 For all the algorithms which gives real-valued embeddings,  we compute the embedding in both $128$ and $256$ dimensions, and report the best result.

\subsection{Reproducibility details for link prediction experiments} 
\begin{comment}
\noindent\textbf{Datasets:}
\texttt{Gowalla}~\cite{snap}:  is a location-based social networking website where users share their locations by checking-in. % The friendship network is undirected and was collected using their public API. 
%The dataset consists of $196,591$ nodes and $950,327$ edges. 
The dataset consist of  a total of $6,442,890$ check-ins of these users over the period of Feb. 2009 - Oct. 2010. \texttt{Enron Emails Network:}~\cite{snap}:  covers all the email communication within a dataset of around half million emails. In this dataset, nodes of the network are email addresses and if an address $i$ sent at least one email to address $j$, the graph contains an undirected edge from $i$ to $j$. 
%The datasets contains $36,692$ nodes and $1,83,831$ edges.
\texttt{BlogCatalog}~\cite{BlogCatalog}:  is the social blog directory which manages the bloggers and their blogs.  
%This dataset is crawled from BlogCatalog webpage \footnote{\url{ http://www.blogcatalog.com}}. 
The dataset contains the friendship network crawled and group memberships. Here, nodes represent users, and edges represent a friendship relation between any two users. 
%The network has $10,312$ nodes and $333,983$ edges. 
In \texttt{Facebook}~\cite{snap} network, nodes represent
users, and edges represent a friendship relation between any
two users. 
%The network has $4,039$ nodes and $88,234$ edges.
\end{comment}

\noindent\textbf{Methodology:} For the purpose of classification, we generate a labeled dataset of edges by splitting a dataset into training and testing partition in $70-30$ ratio. These will serve as our positive training and testing samples. To this purpose, we randomly sample $30\%$ of edges and remove them. During the removal of edges, we make sure that the residual graph obtained after edge removal remains connected. If the sampled edges don't ensure this, we choose a different edge. We learn the embedding of the graph using all the candidate algorithms on our positive training samples. We now generate missing edges equal in number to the original dataset. Missing edges are edges that are absent in the graph. We split the generated missing edges into training and testing partition in $70-30$ ratio, which is  our negative training and testing samples. We compute inner product for all the edges and label them $0$ or $1$ depending on whether it is a missing edge or an actual edge. 
 
 \begin{comment}
 \subsection{Reproducibility details for node classification experiments} 
 \noindent\textbf{Datasets:}
 We used three citation datasets --- \texttt{Cora}, {\tt Citeseer} and \texttt{Pubmed}~\cite{Sen08collectiveclassification} for the experiments. %\footnote{\url{https://linqs.soe.ucsc.edu/data}}. These datasets  are citation networks where nodes
%represent articles and  links represent citations.  
Here, citation relationships are viewed as directed  edges. Attributes associated with nodes are extracted from the title and the abstract of the each article and are presented as sparse bag-of-word vectors, after removing the stop words and low-frequency words. Each article in these datasets has only one label representing the class it belong to. 
We also considered \texttt{IMDB-BINARY}~\cite{YanardagV15,imdb}, 
%\footnote{\url{http://networkrepository.com/IMDB-BINARY.php}}
 which is a movie collaboration dataset where actor/actress and genre information of different movies on IMDB are collected. Nodes represent actors/actresses, and an edge between them signifies a joint appearance in some movie. Collaboration graphs is generated on the ``action'' and the ``romance'' \textit{genres} and derived \textit{ego-networks} for each actor/actress. 
%A movie can belong to both genres at the same time, therefore  movies from romance genre are discarded if they are already included in the action genre. 
Each ego-network is labeled with the genre graph it belongs to. The task is then simply to identify which genre an ego-network graph belongs to.

%Statistics of these datasets, including number of nodes, number of edges, number of classes (categories), and the dimension of attributes are summarised in Table~\ref{tab:data_node_classfication}.  

\end{comment}

 



